Autonomous Artificial Intelligence Agents for Clinical Decision Making in Oncology

Multimodal artificial intelligence (AI) systems have the potential to enhance clinical decision-making by interpreting various types of medical data. However, the effectiveness of these models across all medical fields is uncertain. Each discipline presents unique challenges that need to be addressed for optimal performance. This complexity is further increased when attempting to integrate different fields into a single model. Here, we introduce an alternative approach to multimodal medical AI that utilizes the generalist capabilities of a large language model (LLM) as a central reasoning engine. This engine autonomously coordinates and deploys a set of specialized medical AI tools. These tools include text, radiology and histopathology image interpretation, genomic data processing, web searches, and document retrieval from medical guidelines. We validate our system across a series of clinical oncology scenarios that closely resemble typical patient care workflows. We show that the system has a high capability in employing appropriate tools (97%), drawing correct conclusions (93.6%), and providing complete (94%), and helpful (89.2%) recommendations for individual patient cases while consistently referencing relevant literature (82.5%) upon instruction. This work provides evidence that LLMs can effectively plan and execute domain-specific models to retrieve or synthesize new information when used as autonomous agents. This enables them to function as specialist, patient-tailored clinical assistants. It also simplifies regulatory compliance by allowing each component tool to be individually validated and approved. We believe, that our work can serve as a proof-of-concept for more advanced LLM-agents in the medical domain.

==> Manuscript/pseudoalgo_main_2.tex <==
\newcommand{\customindent}[1]{\hspace{#1}}
\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}

\DeclareMathOperator*{\argmax}{arg\,max}

\begin{algorithm}
\caption{%
    Response generation algorithm.
    This algorithm generates a the model's final response after the agent has invoked the necessary tools in response to the question.
    It involves several calls to the LLM which are denoted as functions of the form \texttt{Generate*($\cdot$)}; these functions invoke the LLM with a templated prompt into which the input arguments are inserted. CoT = Chain-of-Thought, P = Predict (akin to dspy.Predict).
}
\begin{algorithmic}[1]
    \Require
        \Statex Patient context $C_\textit{patient}$ \Comment{Contains clinical information about the patient}
        \Statex Question $Q$ \Comment{Question(s) or instruction(s) related to the patient}
        \Statex Agent tools $A_\textit{tools}$ \Comment{List of all available tools}
        \Statex Tool outputs $T_\textit{out}$ \Comment{Free-text summary of the results of the tools used by the agent}
        \Statex Documents $D$ \Comment{Collection of medical documents (guidelines, textbooks, etc.)}
    \Ensure Comprehensive and accurate response $R$
    \State $C_Q \gets \text{empty list}$ \Comment{Question context (will contain passages relevant to $Q$)}
    \State $\textit{Subqueries} \gets \texttt{GenerateSubqueries}_{\text{CoT}}(C, Q, T_{\text{out}})$ \Comment{Generate 10-14 sub-questions for RAG}
    \ForEach{subquery $q$ \textbf{in} $\textit{Subqueries}$}
        \State $P \gets \text{Retrieve}_n(D, q)$ \Comment{Retrieve $n=40$ passages relevant to the subquery $q$}
        \State $P \gets \text{Rerank}(P, q)$ \Comment{Re-rank the retrieved passages based on relevance to $q$}
        \State $P \gets \text{Top}_k(P)$ \Comment{Keep only the top $k=10$ passages}
        \State $C_Q \gets C_Q \cup P$ \Comment{Add the passages to the question context}
    \EndFor
    \State $C_Q \gets \text{Deduplicate}(C_Q)$ \Comment{Remove duplicate passages}
    \For{$i$ \textbf{in} $1, \dots, |C_Q|$}  \Comment{Add numbered source information to each passage}
        \State $C_Q[i] \gets \text{Concat}(\text{``Source "}, i, C_Q[i])$
    \EndFor
    \State $\textit{Strategy} \gets \texttt{GenerateAnswerStrategy}_{\text{CoT}}(C, Q, A_\textit{tools}, T_\textit{out}, C_Q)$
    \State $\textit{CitedResponse} \gets \texttt{GenerateCitedResponse}_{\text{P}}(C, Q, A_\textit{tools}, T_\textit{out}, C_Q, \textit{Strategy})$
    \State $\textit{Suggestions} \gets \texttt{GenerateSuggestions}_{\text{CoT}}(\textit{CitedResponse}, A_\textit{tools}, T_\textit{out})$
    \State $R \gets \text{Concat}(\textit{CitedResponse}, \textit{Suggestions})$ \Comment{Final output}
    \State \Return $R$
\end{algorithmic}
\end{algorithm}
\setcounter{footnote}{0}

